Preserve, Promote, or Attack? GNN Explanation via Topology Perturbation

Prior works on formalizing explanations of a graph neural network (GNN) focus on a single use case - to preserve the prediction results through identifying important edges and nodes. In this paper, we develop a multi-purpose interpretation framework by acquiring a mask that indicates topology perturbations of the input graphs. We pack the framework into an interactive visualization system (GNNViz) which can fulfill multiple purposes: Preserve,Promote, or Attack GNN's predictions. We illustrate our approach's novelty and effectiveness with three case studies: First, GNNViz can assist non expert users to easily explore the relationship between graph topology and GNN's decision (Preserve), or to manipulate the prediction (Promote or Attack) for an image classification task on MS-COCO; Second, on the Pokec social network dataset, our framework can uncover unfairness and demographic biases; Lastly, it compares with state-of-the-art GNN explainer baseline on a synthetic dataset.

==> visualization.tex <==
\section{{{\GNNViz}}:An Interactive Visualization system and qualitative Visual Analytics}

%\vspace*{-0.05in}
\subsection{System Overview}
%\vspace*{-0.05in}
% %\begin{figure*}[htb]
% %
% {\begin{wrapfigure}{r}{60mm}
% \vspace*{-0.0in}
% \centerline{
% \begin{tabular}{c}
% \includegraphics[width=0.22\textwidth,height=!]{fig/system-UI-topdown.png}
% %\footnotesize{(a)} &   \footnotesize{(b)}
% \end{tabular}}
% \caption{{The User Interface of {\GNNViz}. It has two views: a browser view (TOP), and a detailed view for a single data instance (BOTTOM). 
% }}
% \label{fig:system-ui}
% \vspace*{-0.00in}
% %\end{figure*}
% \end{wrapfigure}
% }%
{\GNNViz} is not only an explanation algorithm but also an interactive, multi-purpose visualization system for interpreting GNN models, as shown in Fig.\ref{fig:system-ui}. In general, it has two user views: a browser view (Fig.\ref{fig:system-ui} \textbf{Top}), and a detailed view (Fig.\ref{fig:system-ui} \textbf{Bottom}).

\paragraph{Browser View} The browser view is the landing page for a user. It consists with three main sections: a filter (Fig.\ref{fig:system-ui} \textbf{A}) that allows a user to specify the filtering condition based on the images' ground truth labels; a navigation list (Fig.\ref{fig:system-ui} \textbf{B}) that allows users to browse all the data instances; and a graph canvas (Fig.\ref{fig:system-ui} \textbf{C}) that presents the global graph learned from the entire dataset, which is agnostic to individual data instances.

The main function of the browser view is to allow a user to quickly navigate through a large amount of data instances and identify the data instances that may be of interest to the user. As shown in Fig.\ref{fig:system-ui} \textbf{B}, the list contains each image, and its groundtruth labels and the targeted GCN algorithm~\cite{Chen2019MultiLabelIR} predicted labels. Noted that the targeted GCN algorithm can have incorrect predictions. For example, in the presented image example in (Fig.\ref{fig:system-ui} \textbf{B}), GCN failed to predict the chair label, but add an extra bench label, when compared to the groundtruth labels. Different user groups may have different user needs for interpretation, thus the system allows each individual user to choose which data instances may be more of interest to them. For example, an non-expert model user may be interested in understanding only the correct prediction cases, thus he or she can click on the images that have an accurate prediction result; whereas an expert GNN model builder may want to understand why the examined GCN algorithm always fails to predict certain labels, thus he or she can click on those images to explore further details. 

The filter function in Fig.\ref{fig:system-ui} \textbf{A} is to further ease such user navigation. In the demonstrated MS-COCO dataset, there are hundreds of thousands image data instances, and it is really hard for a user to manually browse through all the images, thus they can use the filter function to limit the UI to show only a subset of images based on their groundtruth labels. The filter function also support AND operation when a user enters more than one label as the filtering criteria, thus it can further helps users to navigate through large datasets like the demonstrated MS-COCO.

The majority space of the browser view UI is dedicated to the global graph topology. As explained in the previous section, we use a well-cited GCN-based multi-label classification algorithm~\cite{Chen2019MultiLabelIR} as the target model for explanation, and demonstrate our interpretation algorithm and the {\GNNViz} system, despite the interpretation algorithm and {\GNNViz} system are applicable to other GNN algorithms and datasets. The global graph topology map in this case is calculated from the label co-occurence probability from the entire training dataset, as shown in Fig.~\ref{fig:gcn-graph}. Thus, each node in the graph represents a label, and each directed edge represents an co-occurence relationship. The edges are binary, with a threshold of conditional probability at 0.4, as suggested by the original paper. 

This global graph topology can be considered as equivalent to a knowledge graph that contains the domain knowledge of the MS-COCO dataset. By nature, this knowledge graph is agnostic to individual data instances. In the original paper~\cite{Chen2019MultiLabelIR}, the authors only presented an illustrative graph with 5 nodes (Fig. \ref{fig:gcn-graph}). {\GNNViz} presents the entire graph topology with all 80 labels as nodes. The color of nodes are defined by the node categories in the MS-COCO dataset. For example, bird, giraffe, cow and a few other nodes are colored in blue as they all belong to the animal category; and the sport category nodes (baseball bat, skateboard, frisbee, etc) are colored in light green.

The layout of this graph (Fig.~\ref{fig:system-ui} \textbf{C}) uses a force-directed graph layout~\cite{fruchterman1991graph} and the implementation uses a D3.js javascript library~\cite{bostock2011d3}. The rendering algorithm first identifies the central node by calculating the graph's centrality and the degree of the nodes (person node in this case), then distribute other nodes based on their connectivity to the central nodes and their degrees. The disconnected nodes are automatically pushed to the peripheral areas. This global graph is the foundation of the targeted GCN algorithm for interpretation, and it can already convey some meaningful information, such as the oven, refrigerator, toaster and other kitchen appliance are often appear together in an image, whereas giraffe or bear is often alone in an image in the MS-COCO dataset.

\paragraph{Detailed View} After navigating through the browser view (Fig.\ref{fig:system-ui}Top) and identifying a particular image of interest, a user can go to an image's detailed view (Fig.\ref{fig:system-ui}Bottom) by clicking on that image. The detailed view has four major areas, in addition to the selected raw image: the groundtruth label and the GCN prediction result (Fig.\ref{fig:system-ui}\textbf{D}), the updated prediction results (Fig.\ref{fig:system-ui}\textbf{E}) after the user apply one of the three user actions (i.e., \texttt{preserve}, \texttt{promote}, and \texttt{attack} modes), a user control panel that a user can switch between the three user actions and manipulate hyperparameters (Fig.\ref{fig:system-ui}\textbf{F}), and the graph topology canvas ((Fig.\ref{fig:system-ui}\textbf{G})). 

The default user mode is \texttt{preserve} mode, which is not shown in Fig.\ref{fig:system-ui}. The \texttt{preserve} mode falls into the factual explanation use case -- the explanation algorithm identifies a less complex subgraph for prediction, but still try to maintain the best prediction performance as using the original global graph topology. In the user control panel (Fig.\ref{fig:system-ui}\textbf{F}), users can adjust the percentile range selector to revise how many edges they want to keep in the subgraph, which will further impact the \texttt{updated prediction} results in Fig.\ref{fig:system-ui}\textbf{E}. The less edges a user keeps in the subgraph, the worse updated prediction result is. By default, the algorithm identify the subgraph with 10 edges. All rest of the unpreserved edges are shown in a 10\% opacity in the background. In the following visual analytics subsection, we will present more details of this \texttt{preserve} explanation mode.

The second user mode is \texttt{promote} mode, and it is illustrated in Fig.\ref{fig:system-ui}. The \texttt{promote} mode is also for the factual explanation user scenario. For the targeted GNN prediction algorithm (GCN from ~\cite{Chen2019MultiLabelIR} in this case), our {\GNNViz} algorithm can suggest new edges to add into the graph topology and promote the correct prediction results. In the control panel in Fig.\ref{fig:system-ui}\textbf{F}, a user can adjust the progress bar at the bottom to decide how many additional edges they want the {\GNNViz} algorithm to suggest. For example, in Fig.\ref{fig:system-ui}\textbf{Bottom}, the user sets the parameter to two edges for addition. In Fig.~\ref{fig:system-ui}\textbf{G}, the suggested two edges appears in green dash lines (chair to sandwich and chair to wine glass). If a user agrees with the recommendation and wants to explore this suggestion, they can simply click on the green dash lines in Fig.~\ref{fig:system-ui}\textbf{G} to add those edges into the graph topology. The GCN prediction algorithm will recalculate the prediction result using this manipulated graph topology, and the prediction results will be updated in Fig.~\ref{fig:system-ui}\textbf{E}. By default, \texttt{promote} suggests one edge to add. Later in the visual analytics subsection, we will showcase the effectiveness of the proposed {\GNNViz} algorithm with a few data instances.

The third user mode is \texttt{attack} mode. In contrary to the previous two user modes, this mode is to visualize the counterfactual explanation user scenarios. {\GNNViz} can recommend the minimal edge changes (both edge addition and deletion) to attack the GCN prediction algorithm -- manipulate the updated prediction results to move away from the correct predictions. The user interface looks similar to the \texttt{promote} mode shown in Fig.~\ref{fig:system-ui} \textbf{Bottom}. The difference between \texttt{promote} mode and \texttt{attack} mode is that in the graph canvas Fig.~\ref{fig:system-ui} \textbf{G}, the \texttt{attack} mode hide the entire graph topology in the background and highlight only the edges recommended for attacking. It uses green dash lines to indicate the edge addition, and uses red solid lines to indicate edge removal, as shown in Fig.~\ref{fig:subgraphs}.

In summary, the proposed {\GNNViz} system provides an easy-to-use and interactive visualization system for both graph-based model experts and non-technical model users to visually interpret, analyze, and attack GNN models. The implemented three modes--\texttt{preserve, promote, and attack}--satisfy both the factual explanation use case and the counterfactual explanation use case. The visualization system architecture is implemented as a general purpose API-based web service, thus researchers can easily switch the interpretation backend to their own interpretation algorithms and visually interpret its usefulness. Also, if the researcher is not interested in GNN interpretation research topic, the visualization system can simply be used to examine a graph-based model's prediction performance at the instance level. 


%\begin{wrapfigure}{r}{60mm}
\begin{figure*}[h]
\vspace*{-0.0in}
\centerline{
\begin{tabular}{c}
\includegraphics[width=0.99\textwidth,height=!]{fig/subgraphs.png}
%\footnotesize{(a)} &   \footnotesize{(b)}
\end{tabular}}
\caption{{Each row represents one data instance and its \texttt{preserve} mode, \texttt{promote} mode, and \texttt{attack} mode.}}
\label{fig:subgraphs}
\vspace*{-0.2in}
\end{figure*}
%\end{wrapfigure}

%\vspace*{-0.05in}
\subsection{Qualitative Visual Analytics}
%\vspace*{-0.05in}

As noted in the previous subsection, the model builders and model users can use the {\GNNViz} visualization system to interpret why a graph-based model produces certain predictions, both correct and incorrect ones. This is considered as the factual explanation use case. In addition, there is also a counterfactual explanation use case. That some other users may be more interested in the adversarial robustness of a graph-based model, thus they want to identify the vulnarability points of a GNN model through attacking its graph topology. In this section, we will use a few examples (Fig.\ref{fig:subgraphs}) to illustrate how our implemented {\GNNViz} algorithm and visualization system support both use cases.

As shown in Fig.\ref{fig:subgraphs}, we present four image data instances (each in a row) and their three modes (each in a column). In the first column, we present the raw image, its groundtruth label, and its prediction result generated by the GCN model~\cite{Chen2019MultiLabelIR} that {\GNNViz} aims to explain. Sometimes the GCN prediction model may generate incorrect predictions. For example, in the second row of the data, the GCN model fails to predict the \texttt{Handbag} label, but mis-predicts an extra \textit{Car} label. For the labels that GCN correctly predicts, a user may be interested to know why the graph-based model makes such correct prediction; for the incorrect labels, a user may want to know why the model makes a wrong prediction. These user needs are categorized as \textbf{factual explanation} use cases, and we design a \texttt{Preserve} mode and a \texttt{Promote} mode for it. In addition, a user may wants to increase the robustness of a graph-based model, thus he or she needs to identify the adversarial vulnerability of the graph topology--where in the graph a user can spent the minimal effort to change the edges and to negatively impact the prediction result. We treat this use case separately as a \textbf{counterfactual explanation} need and design the \texttt{Attack} mode for it. 

In summary, we will use the rest of this subsection to illustrate how {\GNNViz} visualization system can help a user to understand, improve, and attack a model's prediction outcome by examining and interacting with the visual graph topology. 

\paragraph{How does the graph topology contribute to a graph-based model's correct or incorrect prediction results?}

In the \texttt{preserve} mode, our interpretation algorithm preserves a sparse subgraph (by default ten-edges) to reduce the complexity while still maintaining a relative good performance. By looking only at the raw images column and the \texttt{preserve} mode column, we can see that for the data instance (1), the \texttt{preserve} mode subgraph successfully captures the most important edge \texttt{Person}--to--\texttt{Motorcycle} in the topology, because the \texttt{Person}--to--\texttt{Motorcycle} link is the thickest one. But the GCN model fails to predict \texttt{Bird}, \texttt{Bagpack} or \texttt{Handbag}, as these edges are not in the top-ten edges in the preserved subgraph.

In contrary, we can see from the second data instance (2) that the GCN model mis-predicts the \texttt{Car} label. And the preserve subgraph reflects such misprediction as it believes the \texttt{Person}--to--\texttt{Car} edge has a high importance level. The model builder can further dive into the graph topology and the CNN classifier to examine why this mistake happens. 

\paragraph{How to improve a graph-based model's prediction performance?}
In the \textit{promote} mode, our interpretation algorithm suggests new edges to add to the graph to improve the prediction correctness. Worth to mention, the promote mode is targeting the global graph topology, instead of the preserved subgraph. The user can click on the suggested edges in the subgraph in the \textit{promote} mode and the selected edges will be added onto the graph topology, and the prediction probabilities will be recalculated and updated. By default and as illustrated in Fig.\ref{fig:subgraphs}, we set the parameter to allow {\GNNViz} algorithm to suggest only one edge to add, but the user can use the control panel in Fig.\ref{fig:system-ui}\textbf{F} to interactively change such setting. 

For example, for the fourth data instance, the GCN model fails to predict \texttt{Banana} and \texttt{Orange}. As shown in the \texttt{Promote} mode, the {\GNNViz} algorithm correctly suggest to add a \texttt{Banana}--to--\texttt{Apple} link. And if the user agrees with such suggestion and clicks on that edge in the subgraph, the GCN model will recalculate the prediction result and successfully predict the \texttt{Banana} and \texttt{Orange} labels, while not affecting other labels.


\paragraph{How to attack a graph-based model?}
In the \texttt{attack} mode, the interpretation algorithm can suggest both edges to be added and edges to be deleted. The attack mode also targets the global graph topology, thus the edges to be added or to be deleted are selected from the global graph. We use the green dash line to indicate the edges suggested to add, and the red solid line to indicates the edges to be removed. By default, we set the parameter for {\GNNViz} algorithm to suggest only one edge to add and one edge to remove, but the user can change this hyperparameter in the control panel via the UI.

As shown in the first data instance, the GCN model initially correctly predicts \texttt{Motrocycle} and \texttt{Person}. The {\GNNViz} algorithm suggests to add the \texttt{WineGlass}--to--\texttt{Motorcle} link and remove the \texttt{Bench}--to--\texttt{Person} link from the graph topology. If the user applies such suggestions, the GCN model will recalculate the prediction result and mistakenly believes \texttt{Kite} is the top prediction label. Similarly, in the third data instance row, if the user agrees with the algorithm suggestion by adding \texttt{Spoon}--to--\texttt{BaseballBat} and removing \texttt{Bowl}--to--\texttt{Person} edges, the GCN model can not predict the \texttt{Person} label anymore, and the attack is successful.
% \footnote{Note that for some other data instances, it is possible that it needs the {\GNNViz} algorithm to suggest more-than-one edge changes to make the attack successful.}

